AccentCanvas: Activity-Guided Bidirectional Accent Conversion

Accent conversion for dubbing must change pronunciation while preserving content, voice, and source timing. Normalization alone cannot produce requested non-native accents, and matching total duration does not ensure local speech/pause alignment. We present AccentCanvas, a shared discrete diffusion model for normalization and L1-to-L2 conversion, trained on cross-paired shared-prompt recordings and synthetic pairs. Frame-level speech activity and repetition-preserving units guide local timing through synthesis. Across both tasks, AccentCanvas achieves the highest accent conversion performance (Accent Arrival) and mean listener-rated accent similarity among compared systems, with over 73% lower speech-boundary error than the best baseline for each task. These gains accompany higher L1-to-L2 WER than TokAN and Vevo-Style, highlighting a tradeoff between requested-accent resemblance and ASR-based content recognition. https://smokedindia.github.io/accentcanvas/

==> tables/02_human.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{4pt}
\caption{Planned listening evaluation; all values are pending.
MOS-N rates naturalness; XAB measures preference for the row system against a comparator using an independent target-accent reference.
Instruments, comparators, and sample sizes remain to be set.}
\label{tab:human}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcc@{}}
\toprule
System & MOS-N $\uparrow$ & XAB (\%) $\uparrow$ \\
\midrule
\multicolumn{3}{l}{\textbf{Normalization: L2 $\to$ native}} \\
\our{} (base) & TBD & TBD \\
\our{} & TBD & TBD \\
\midrule
\multicolumn{3}{l}{\textbf{L1-to-L2: native $\to$ L2}} \\
\our{} (base) & TBD & TBD \\
\our{} & TBD & TBD \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/archive/table_groups.tex <==
\begin{table*}[t]
\centering\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{10pt}
\caption{Available-group arrival by evaluated cell under the primary reference cap. Removal columns denote source groups and installation columns denote requested target groups. Counts after reference exclusions are shown in the headings. Other L2 labels serve as distractor references, not evaluated conversion targets.}
\label{tab:groups}
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{Removal: requested native} & \multicolumn{3}{c}{Installation: source native} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
System & Arabic (39) & Hindi (38) & Korean (38) & Hindi (40) & Korean (40) & Mandarin (40) \\
\midrule
Base (Whisper-DiT) & 0.744 & 0.842 & 0.842 & 0.325 & 0.125 & 0.125 \\
LT+Cosy25 (seed 1) & 0.718 & 0.921 & 0.895 & 0.225 & 0.100 & 0.075 \\
LT+Cosy25 (seed 2) & 0.718 & 0.895 & 0.789 & 0.250 & 0.125 & 0.075 \\
TokAN & 0.641 & 0.763 & 0.921 & -- & -- & -- \\
TokAN L1$\to$L2 (reprod.) & -- & -- & -- & 0.000 & 0.100 & 0.025 \\
CosyAccent & 0.615 & 0.921 & 0.921 & -- & -- & -- \\
CosyAccent-segmentwise & 0.436 & 0.816 & 0.632 & -- & -- & -- \\
RWA & 0.308 & 0.684 & 0.605 & 0.075 & 0.075 & 0.050 \\
Vevo-Style & 0.333 & 0.632 & 0.684 & 0.050 & 0.000 & 0.050 \\
\midrule
Source-unit resynthesis & 0.128 & 0.289 & 0.395 & 0.000 & 0.025 & 0.000 \\
Real-target-unit resynthesis & 0.949 & 0.947 & 0.974 & 0.300 & 0.275 & 0.325 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/archive/table_robustness.tex <==
\begin{table}[t]
\centering\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{5pt}
\caption{Sensitivity of arrival to the maximum reference count. Native pools remain smaller than L2 pools on many prompts, including under cap 2; this is not an equal-pool control.}
\label{tab:robustness}
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{Removal} & \multicolumn{2}{c}{Installation} \\
System / control & Cap 3 & Cap 2 & Cap 3 & Cap 2 \\
\midrule
Base & 0.809 & 0.783 & 0.192 & 0.200 \\
LT+Cosy25, seed 1 & 0.843 & 0.791 & 0.133 & 0.167 \\
LT+Cosy25, seed 2 & 0.800 & 0.757 & 0.150 & 0.192 \\
Source units & 0.270 & 0.287 & 0.008 & 0.008 \\
Target units & 0.957 & 0.922 & 0.300 & 0.250 \\
\bottomrule
\end{tabular}
\end{table}

